From RAN Control to Agentic Intelligence: Architecture and Vision for Energy Efficient AI-RAN

Future 6G networks will rely on highly distributed, AI-native Radio Access Networks (RANs), where communication and AI workloads share a common infrastructure. This evolution, combined with increasing deployment density and continuous AI processing, is expected to significantly increase RAN energy consumption. While Open RAN (O-RAN) introduces a programmable and modular control framework through the RAN Intelligent Controller (RIC) and Service Management and Orchestration (SMO), current approaches remain largely policy-driven, limiting adaptive energy-aware coordination across multiple applications. In parallel, AI-RAN promotes the convergence of AI and RAN infrastructures through AI-for-RAN, AI-on-RAN, and AI-and-RAN paradigms, yet efficient mechanisms to jointly orchestrate performance, latency, and energy remain an open challenge. This article proposes an agentic AI-native RAN architecture that bridges O-RAN's structured control with AI-RAN's unified vision. Leveraging semantic intent abstraction and Large Language Model (LLM)-driven coordination, the framework enables adaptive orchestration, conflict resolution, and energy-aware multi-objective optimization across heterogeneous workloads. Through representative AI-for-RAN and AI-on-RAN use cases, we show how such coordination can improve resource efficiency and reduce operational energy consumption, paving the way toward sustainable 6G networks.

==> sections/UseCases.tex <==
%Intent → reasoning → action loop

\subsection{Use Cases: From Intent to rApp-Level Control}

We illustrate the proposed orchestration loop through two complementary use cases. The objective is not to claim that the LLM directly computes radio-control actions, but to show how specialized rApps can be exposed to an LLM-based manager through natural-language intents, operational meta-parameters, validation hooks, and KPI feedback.

For both use cases, the operator intent can be expressed as: "reduce RAN energy consumption while preserving service quality and user experience." The LLM-based manager interprets this intent and produces a structured orchestration plan. This plan specifies which rApp should be used, what inputs are required, which operational constraints must be enforced, and which meta-parameters should be selected or validated through the Digital Twin.

\subsubsection{AI for RAN: Prediction-Based Sector Carrier Steering}

The first use case corresponds to AI for RAN, where AI is used to optimize the operation of the RAN itself. The intent is network-centric: reduce radio energy consumption while preserving sector capacity and service quality. The selected control function is a prediction-based sector steering rApp.

This rApp receives predicted sector PRB demand, the current active carrier set, per-carrier PRB capacities, and operational constraints such as the always-on anchor coverage carrier and a maximum load threshold. Its role is to select the minimum set of active carriers able to serve the predicted demand without violating capacity and quality constraints. The LLM does not compute this carrier decision directly. Instead, it provides operational meta-parameters, such as the energy-saving profile, the load threshold, the prediction horizon, and the stability guard. These parameters can be selected from configurations previously evaluated offline or through the Digital Twin.

The rApp then generates candidate active-carrier configurations and reports their expected energy gain and service-quality impact. These candidate configurations are evaluated by the Digital Twin, which checks traffic evolution, capacity limits, QoS requirements, and operational constraints before deployment. The Energy Efficiency Agent can further assess the energy--performance trade-off. Only validated configurations are applied in the RAN. This follows the sector-level carrier steering logic, where predicted sector demand is used to keep only the necessary active capacity while preserving the coverage carrier and QoS safeguards~\cite{abbar:hal-05627005}.

\subsubsection{AI on RAN: UX-Aware DRL Steering for Edge AI Services}

The second use case illustrates AI on RAN. In this case, the RAN is not only optimized as a communication system, but also supports latency-sensitive AI services deployed close to the users at the network edge. Such services may include real-time inference or interactive AI applications, where user experience depends on both radio conditions and edge-service performance.

The application-level requirements are provided through the Application Controller and the Enrichment Database, for example latency sensitivity, service priority, UX target, and energy constraints. Based on this information, the LLM-based manager can select a UX-aware DRL steering rApp and provide meta-parameters such as the UX target profile, the energy-saving aggressiveness, and the service-degradation penalty profile.

The DRL rApp receives the network state, including per-carrier PRB load, number of users, throughput or UX-related KPIs, and carrier states. It outputs a carrier ON/OFF action and a user reallocation decision among the remaining active carriers. This rApp acts as the RAN-side control function supporting the AI-on-RAN scenario: the edge AI service exposes UX or latency requirements, and the DRL rApp adapts carrier shutdown and user reallocation so that energy saving does not degrade the service experience. Candidate actions are validated through the Digital Twin, which checks both network constraints and service-level requirements, while the Energy Efficiency Agent evaluates the energy--QoE trade-off. Only actions satisfying both network and edge-service constraints are executed. The DRL rApp has been shown to reduce energy consumption while maintaining UX guarantees by jointly deciding carrier shutdown and user reallocation~\cite{11044545}.

\begin{table*}[!t]
\centering
\caption{Intent-to-rApp orchestration outputs for the two illustrative use cases.}
\label{tab:metaparameters}
\begin{tabular}{p{0.22\linewidth} p{0.28\linewidth} p{0.34\linewidth}}
\toprule
\textbf{Use case} & \textbf{Intent} & \textbf{LLM/Digital Twin orchestration output} \\
\midrule
AI for RAN: sector steering &
Reduce RAN energy while preserving sector capacity and service quality. &
Deploy the prediction-based sector steering rApp; enforce the always-on anchor carrier and maximum load constraint; select the activation/deactivation threshold profile, prediction horizon, and stability guard; validate candidate configurations through the Digital Twin and Energy Efficiency Agent. \\
\midrule
AI on RAN: UX-aware DRL steering &
Reduce energy while preserving the UX of an edge AI service deployed close to users. &
Deploy the UX-aware DRL steering rApp; enforce service-continuity and UX constraints; select the UX target profile, energy-saving aggressiveness, and service-degradation penalty profile; validate candidate actions through the Digital Twin and Energy Efficiency Agent. \\
\bottomrule
\end{tabular}
\end{table*}

The deployment trigger is also part of the orchestration output. When the ecological intent is active and the Digital Twin validates that an energy-saving profile can satisfy the required service-quality constraints, the corresponding rApp is deployed or configured. Otherwise, the system keeps a safer profile, such as the All-ON configuration or a less aggressive energy-saving mode.

After execution, each rApp reports its gains and KPI impact through the performance-management loop. This feedback is then used by the LLM-based manager to decide whether to keep the same configuration, relax the energy-saving policy, or switch to a safer profile. If candidate actions conflict, the Digital Twin/Validator Agent checks feasibility first, while hard constraints such as coverage, maximum load, service continuity, and UX preservation take priority over energy saving.


==> sections/evaluation.tex <==
\section{Performance Evaluation}
\label{sec:performance}

This section illustrates how the proposed LLM-based orchestration loop is instantiated with two energy-efficiency rApps. The LLM-based manager produces the orchestration plan and selects the operational profiles, while the specialized rApps compute the radio-control actions and report the resulting KPIs. The objective is therefore not to benchmark the LLM as a standalone algorithm, but to show how LLM-guided orchestration can rely on rApp-level KPI feedback.

\subsection{Simulation Setup}

We consider a sector-level carrier steering setting. A radio site is typically divided into directional sectors, each serving users in a given geographical area. Within one sector, several co-located carriers operate on different frequency bands and jointly provide coverage and capacity. The carrier steering decision is therefore taken at the sector level: depending on traffic demand and service-quality constraints, some carriers may remain active while others may be temporarily put into sleep mode.

For the illustration, both rApps are presented under a unified five-carrier sector template with carriers at 700, 800, 1800, 2100, and 2600 MHz. The 700 MHz carrier is always kept active as the anchor coverage layer. The 800 MHz carrier is a low-band controllable layer that contributes to coverage robustness, while the 1800, 2100, and 2600 MHz carriers mainly provide additional capacity. This representation is used only to provide a common orchestration view across the two rApps: active carrier configuration, energy gain, service-quality feedback, and constraint satisfaction.

The reported results are obtained over a one-month trace window with 15-minute decision granularity. The same number of sector instances is retained for the two rApp illustrations, so that the KPI feedback is presented at the same aggregation level. The All-ON configuration, where all carriers remain active, is used as the reference operating mode.

\subsection{Compared Profiles and Metrics}

The baseline is the All-ON configuration. It is the safest operating mode from a service-quality perspective, but it provides no energy saving.

For each use case, we instantiate the same orchestration pattern: an operator intent is translated by the LLM-based manager into an orchestration output validated through the Digital Twin, including the rApp to deploy and the operational profile to use. The selected rApp profile is then evaluated on one-month network traces, and the resulting KPIs are reported as feedback to the orchestration layer. The selected profiles correspond to configurations that provide a favorable trade-off between energy gain and service-quality preservation.

For the AI-for-RAN use case, the considered intent is to reduce sector energy consumption while preserving the anchor coverage layer and maintaining throughput satisfaction. The LLM/Digital Twin orchestration output is the deployment of the prediction-based sector steering rApp with selected activation/deactivation threshold profiles. The rApp then returns the active carrier configuration, energy gain, coverage satisfaction, and throughput satisfaction.

For the AI-on-RAN use case, the considered intent is to reduce energy while preserving the UX of an edge AI service. The assumed LLM/Digital Twin output is the deployment of the UX-aware DRL steering rApp with selected UX target and service-degradation penalty profiles. The rApp then returns the carrier ON/OFF action, user reallocation decision, energy gain, UE satisfaction, and UX satisfaction.

The reported metrics correspond to the KPI feedback that would be made available to the orchestration layer. \emph{Energy gain} measures the energy reduction with respect to the All-ON baseline. \khoa{\sout{\emph{Coverage/UE satisfaction} captures the safety-related constraint: coverage preservation for the prediction-based sector steering rApp, and UE service-continuity satisfaction for the DRL-based rApp.}} \khoa{\emph{Coverage satisfaction}} captures the safety-related constraint of both rApp: preservation of service and connectivity. \emph{Throughput satisfaction} reports the retained throughput quality for the prediction-based rApp. \khoa{\emph{UX-5} and \emph{UX-10 satisfaction} measure how consistently the UX is met for at least 95\% and 90\% of users, respectively.} Separate violation counters are not shown; violations are reflected by satisfaction indicators below 100\%.


Figure~\ref{fig:rapp_results} shows that the prediction-based sector steering rApp reaches energy gains of 16\% and 19\% for the two selected profiles, while preserving coverage and maintaining high throughput satisfaction. The UX-aware DRL rApp reaches energy gains of 15\% and 18\%, while reporting UE and UX satisfaction indicators. These results should be interpreted as representative rApp-level outputs: they illustrate the type of feedback that the proposed LLM-based manager can use to compare candidate profiles, adjust meta-parameters, or trigger validation through the Digital Twin.

==> sections/useCase2.tex <==

\subsubsection{AI for RAN: Prediction-Based Sector Carrier Steering}
\textcolor{red}{
The first use case corresponds to AI for RAN, where AI is used to optimize the operation of the RAN. The operator intent is to reduce RAN energy consumption while preserving sector capacity and quality of service.}

\textcolor{red}{
In this context, a prediction-based sector steering rApp is exposed as an AI-for-RAN control function. This rApp receives as input the predicted sector PRB demand, the current set of active carriers, per-carrier PRB capacities, and operational constraints such as the always-on coverage carrier and a maximum load threshold. Its objective is to determine the minimum set of active carriers required to serve the predicted demand without violating capacity and QoS constraints.}

\textcolor{red}{
Within the orchestration loop, the LLM-based SCA does not directly compute the carrier activation decision. Instead, it selects the appropriate rApp and configures it through high-level meta-parameters, such as the energy-saving profile, the load threshold, the prediction horizon, and stability constraints. These meta-parameters reflect the trade-off between energy efficiency and service performance implied by the operator intent.}

\textcolor{red}{
Based on this configuration, the rApp generates candidate carrier activation strategies. These strategies are then evaluated using DT, which simulates traffic evolution and validates constraint satisfaction, including capacity limits, QoS requirements, and operational constraints. This enables the system to assess the feasibility and expected impact of each candidate configuration before deployment.}

\textcolor{red}{
Only configurations validated by the DT are applied, ensuring safe and reliable operation. The rApp further provides estimated KPI impact and energy savings, which can be complemented by the Energy Efficiency (EE) agent to refine decision quality.}

\textcolor{red}{
This use case follows a prediction-driven sector-level steering approach, where future demand is used to dynamically adapt active capacity while preserving coverage and QoS guarantees~\cite{abbar:hal-05627005}. Through this process, E-ARC enables predictive, energy-aware, and constraint-compliant control of RAN resources.}

\begin{figure}[t]
\centering
\begin{tikzpicture}[
    node distance=1.6cm,
    box/.style={
        draw,
        rectangle,
        rounded corners,
        align=center,
        text width=6cm,
        minimum height=1.1cm,
        font=\small
    },
    arrow/.style={->, thick}
]

% Nodes
\node[box] (intent) {\textbf{Operator Intent}\\
Reduce energy by $X\%$ while limiting QoS degradation to $Y\%$\\
($X \leq 20$, $Y \leq 5$)};

\node[box] (sca) [below of=intent] {\textbf{LLM-based SCA}\\
Intent interpretation and conflict resolution\\
rApp selection and configuration\\
Meta-parameters: $T_{\text{off}}, T_{\text{on}},$ load thresholds};

\node[box] (rapp) [below of=sca] {\textbf{Prediction-based rApp}\\
Generate candidate carrier configurations};

\node[box] (dt) [below of=rapp] {\textbf{Digital Twin / Validator}\\
Simulate traffic and validate constraints\\
(Capacity, QoS, load limits)};

\node[box] (ee) [below of=dt] {\textbf{Energy Efficiency Agent}\\
Evaluate energy savings and KPI trade-offs};

\node[box] (exec) [below of=ee] {\textbf{RAN Execution (RIC)}\\
Apply carrier ON/OFF configuration};

\node[box] (fb) [below of=exec] {\textbf{Feedback Loop}\\
KPIs: throughput, QoS, energy};

% Arrows
\draw[arrow] (intent) -- (sca);
\draw[arrow] (sca) -- (rapp);
\draw[arrow] (rapp) -- (dt);
\draw[arrow] (dt) -- (ee);
\draw[arrow] (ee) -- (exec);
\draw[arrow] (exec) -- (fb);

% Feedback loop
\draw[arrow] (fb.east) to[out=0, in=0, looseness=1.2] (sca.east);

\end{tikzpicture}
\caption{E-ARC orchestration workflow for AI-for-RAN sector steering.}
\label{fig:workflow_ai_for_ran}
\end{figure}

\begin{figure}[t]
\centering
\begin{tikzpicture}[
    node distance=4.6cm,
    box/.style={
        draw,
        rectangle,
        rounded corners,
        align=center,
        text width=6cm,
        minimum height=1.1cm,
        font=\small
    },
    arrow/.style={->, thick}
]

% Nodes
\node[box] (intent) {\textbf{Operator Intent}\\
Reduce energy up up X\% while downgrading QoS by y \% 
X <-20 and y <- 5\%
};

\node[box] (sca) [below of=intent] {\textbf{LLM-based SCA}\\
Intent interpretation (Intent conflict resolution)\\
rApp selection \& deployment\\
Meta-parameter configuration\\
traffic threshold for activate or deactivate cells <- 10\% $T_{off}$ <- predicted of PRB /(sum of number of PRB of active cell the whole capacity), $T_{on}$ <- the same 
When we reach the On we go to carrier on overwise we go to o
for  is the \% traffic that the cell will be handling
If you predict we have 100 prb 
};

\node[box] (rApp) [below of=sca] {\textbf{rApp deployment}\\
Generate candidate strategies};

\node[box] (dt) [below of=rapp] {\textbf{Digital Twin / Validator}\\
Simulate traffic and check constraints\\ fine tune the meta-parameters parameter
then we deploy rApp (LLM)};

\node[box] (ee) [below of=dt] {\textbf{Energy Efficiency Agent}\\
Evaluate energy savings and KPI trade-offs};

% \node[box] (valid) [below of=ee] {\textbf{Validated Strategy}};

% \node[box] (exec) [below of=valid] {\textbf{RAN Execution (RIC)}\\
% Apply carrier configuration\\ put the carrier in sleep mode
% };

\node[box] (fb) [below of=exec] {\textbf{Feedback Loop}\\
KPIs: throughput, QoE, energy
\\ the feedback should go to the DT + LLM};

% Arrows
\draw[arrow] (intent) -- (sca);
\draw[arrow] (sca) -- (rapp);
\draw[arrow] (rapp) -- (dt);
\draw[arrow] (dt) -- (ee);
\draw[arrow] (ee) -- (valid);
\draw[arrow] (valid) -- (exec);
\draw[arrow] (exec) -- (fb);

% Feedback loop (clean)
\draw[arrow] (fb.east) to[out=0, in=0, looseness=1.2] (sca.east);

\end{tikzpicture}
\caption{E-ARC orchestration workflow for AI-for-RAN sector steering.}
\label{fig:workflow_ai_for_ran}
\end{figure}


\subsubsection{AI on RAN: UX-Aware DRL Steering over Edge Infrastructure}

\textcolor{red}{
The second use case illustrates AI on RAN, where the RAN operates not only as a communication system but also as a distributed edge computing platform hosting AI services close to end users. In this context, edge nodes colocated with RAN infrastructure execute AI workloads such as real-time inference, XR applications, or AI-driven analytics, requiring strict latency and Quality of Experience (QoE) guarantees.
}

\textcolor{red}{
The objective is to reduce energy consumption while preserving service performance, ensuring that energy-saving actions at the RAN do not degrade the QoE of edge-hosted services. In this scenario, a UX-aware DRL-based steering rApp is exposed as an AI-on-RAN control function.}


\textcolor{red}{
Unlike AI-for-RAN approaches that rely solely on network KPIs, this rApp operates on both network and application-level information. Application and service context, including latency constraints, QoE targets, service priorities, and workload characteristics, is provided through the Enrichment Database, reflecting the requirements of edge-hosted services.}

\textcolor{red}{
The rApp receives as input the network state (e.g., per-carrier PRB load, number of users, throughput) together with application-level constraints retrieved from the Enrichment Database. Based on this information, it generates carrier ON/OFF decisions and user reallocation strategies across the remaining active carriers.}

\textcolor{red}{
Within the orchestration loop, the LLM-based SCA selects the DRL-based rApp and configures it through high-level meta-parameters, such as the target QoE profile, \khoa{\sout{energy-saving aggressiveness}}, and penalty associated with service degradation. These parameters are derived from both operator intents and the requirements of edge-hosted applications, enabling context-aware coordination.}


\textcolor{red}{
The rApp generates candidate control actions, which are evaluated using the Digital Twin (DT). The DT simulates both network dynamics and user-level service performance at the edge, allowing the system to assess the impact of decisions on latency, throughput, and QoE. Application constraints from the Enrichment Database are explicitly incorporated into this validation process, ensuring that edge service requirements are respected.}


\textcolor{red}{
In parallel, the Energy Efficiency (EE) agent evaluates energy savings and their impact on system performance, enabling the selection of strategies that align with sustainability and QoE objectives.}

\textcolor{red}{
Only actions that satisfy both network constraints and edge service requirements are executed, ensuring that energy optimization does not compromise the performance of AI services deployed at the network edge. The resulting decisions are applied in the RAN, and both network KPIs and service-level metrics are fed back into the coordination loop for continuous adaptation.}

\textcolor{red}{
This use case highlights how E-ARC enables joint coordination of communication, computation, and user experience in edge-enabled AI-RAN systems, ensuring energy-efficient operation while preserving service quality.}


\begin{figure*}[t]
\centering
\begin{tikzpicture}[
    node distance=1.6cm,
    box/.style={
        draw,
        rectangle,
        rounded corners,
        align=center,
        text width=6cm,
        minimum height=1.1cm,
        font=\small
    },
    arrow/.style={->, thick}
]

% --- Edge Services (top context) ---
\node[box] (edge) {\textbf{Edge AI Services}\\
XR, AI inference, analytics\\
Latency and QoE constraints};
%%% Reduce RAN energy consumption while preserving the QoE and the Latency of AI services 
%%% the meta parameters are the UX target profile
%reduce the energy consumption up to 20\% while preserving the QoE of an edge-hosted AI service. More specifically, the system should keep service continuity high, and preserve UE satisfaction.

% --- Intent ---
\node[box] (intent) [below of=edge] {\textbf{Operator Intent}\\
Reduce energy while preserving UX};

% --- Enrichment DB ---
\node[box] (db) [right=3.5cm of intent] {\textbf{Enrichment Database}\\
QoE targets, latency constraints,\\
service priorities, workloads};

% --- SCA ---
\node[box] (sca) [below of=intent] {\textbf{LLM-based SCA}\\
Intent interpretation\\
rApp selection\\
Meta-parameter configuration};

% --- rApp ---
\node[box] (rapp) [below of=sca] {\textbf{UX-aware DRL rApp}\\
Carrier ON/OFF + user reallocation};

% --- DT ---
\node[box] (dt) [below of=rapp] {\textbf{Digital Twin / Validator}\\
Simulate network + service performance\\
Check QoE and system constraints};

% --- EE ---
\node[box] (ee) [below of=dt] {\textbf{Energy Efficiency Agent}\\
Evaluate energy savings\\
and QoE/KPI trade-offs};

% --- Valid ---
\node[box] (valid) [below of=ee] {\textbf{Validated decision}};

% --- Execution ---
\node[box] (exec) [below of=valid] {\textbf{RAN + Edge Execution}\\
Apply carrier config + serve users};

% --- Feedback ---
\node[box] (fb) [below of=exec] {\textbf{Feedback Loop}\\
KPIs + QoE + service metrics};

% --- Connections ---
\draw[arrow] (edge) -- (intent);
\draw[arrow] (intent) -- (sca);
\draw[arrow] (sca) -- (rapp);
\draw[arrow] (rapp) -- (dt);
\draw[arrow] (dt) -- (ee);
\draw[arrow] (ee) -- (valid);
\draw[arrow] (valid) -- (exec);
\draw[arrow] (exec) -- (fb);

% --- DB connections ---
\draw[arrow] (db.west) -- (sca.east);
\draw[arrow] (db.west) |- (dt.east);

% --- Feedback loop ---
\draw[arrow] (fb.east) to[out=0, in=0, looseness=1.2] (sca.east);

\end{tikzpicture}
\caption{E-ARC orchestration workflow for AI-on-RAN with edge-aware coordination.}
\label{fig:workflow_ai_on_ran}
\end{figure*}

--------------------------



\begin{figure*}[t]
\centering
\begin{tikzpicture}[
    node distance=1.6cm,
    box/.style={
        draw,
        rectangle,
        rounded corners,
        align=center,
        text width=6cm,
        minimum height=1.1cm,
        font=\small
    },
    arrow/.style={->, thick}
]

% --- Edge Services (top context) ---
\node[box] (edge) {\textbf{Edge AI Services}\\
XR, AI inference, analytics\\
Latency and QoE constraints};

% --- Intent ---
\node[box] (intent) [below of=edge] {\textbf{Operator Intent}\\
Reduce energy while preserving UX};

% --- Enrichment DB ---
\node[box] (db) [right=3.5cm of intent] {\textbf{Enrichment Database}\\
QoE targets, latency constraints,\\
service priorities, workloads};

% --- SCA ---
\node[box] (sca) [below of=intent] {\textbf{LLM-based SCA}\\
Intent interpretation\\
rApp selection\\
Meta-parameter configuration};

% --- rApp ---
\node[box] (rapp) [below of=sca] {\textbf{UX-aware DRL rApp}\\
Carrier ON/OFF + user reallocation};

% --- DT ---
\node[box] (dt) [below of=rapp] {\textbf{Digital Twin / Validator}\\
Simulate network + service performance\\
Check QoE and system constraints};

% --- EE ---
\node[box] (ee) [below of=dt] {\textbf{Energy Efficiency Agent}\\
Evaluate energy savings\\
and QoE/KPI trade-offs};

% --- Valid ---
\node[box] (valid) [below of=ee] {\textbf{Validated decision}};

% --- Execution ---
\node[box] (exec) [below of=valid] {\textbf{RAN + Edge Execution}\\
Apply carrier config + serve users};

% --- Feedback ---
\node[box] (fb) [below of=exec] {\textbf{Feedback Loop}\\
KPIs + QoE + service metrics};

% --- Connections ---
\draw[arrow] (edge) -- (intent);
\draw[arrow] (intent) -- (sca);
\draw[arrow] (sca) -- (rapp);
\draw[arrow] (rapp) -- (dt);
\draw[arrow] (dt) -- (ee);
\draw[arrow] (ee) -- (valid);
\draw[arrow] (valid) -- (exec);
\draw[arrow] (exec) -- (fb);

% --- DB connections ---
\draw[arrow] (db.west) -- (sca.east);
\draw[arrow] (db.west) |- (dt.east);

% --- Feedback loop ---
\draw[arrow] (fb.east) to[out=0, in=0, looseness=1.2] (sca.east);

\end{tikzpicture}
\caption{E-ARC orchestration workflow for AI-on-RAN with edge-aware coordination.}
\label{fig:workflow_ai_on_ran}
\end{figure*}


